Bamboo: Building Mega-Scale Vision Dataset Continually with Human-Machine Synergy

Large-scale datasets play a vital role in computer vision. But current datasets are annotated blindly without differentiation to samples, making the data collection inefficient and unscalable. The open question is how to build a mega-scale dataset actively. Although advanced active learning algorithms might be the answer, we experimentally found that they are lame in the realistic annotation scenario where out-of-distribution data is extensive. This work thus proposes a novel active learning framework for realistic dataset annotation. Equipped with this framework, we build a high-quality vision dataset -- Bamboo, which consists of 69M image classification annotations with 119K categories and 28M object bounding box annotations with 809 categories. We organize these categories by a hierarchical taxonomy integrated from several knowledge bases. The classification annotations are four times larger than ImageNet22K, and that of detection is three times larger than Object365. Compared to ImageNet22K and Objects365, models pre-trained on Bamboo achieve superior performance among various downstream tasks (6.2% gains on classification and 2.1% gains on detection). We believe our active learning framework and Bamboo are essential for future work.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/1.Abstract.tex <==
\begin{abstract}
Large-scale datasets play a vital role in computer vision. Existing datasets are collected according to heuristic label systems and annotated blindly without differentiation to samples, making the data collection inefficient and unscalable. How to actively collect, annotate and build a mega-scale dataset is an open question.
%
We found that though we can solve this question by advanced active learning, those typical active learning methods lame in---ineffective than random sampling---the realistic annotation scenario where out-of-distribution data is extensive in the unlabeled pool.
%
In this work, we systematically solve this problem for the classification and detection annotation, proposing a novel active learning pipeline that is effective than random sampling dramatically. 
%
Equipped with this pipeline, we build a high-quality vision dataset---\textbf{\Datasetname}, consisting of 69M image classification annotations and
28M object bounding box annotations. 
%
Compared to ImageNet22K and Objects365, models pre-trained on \Datasetname~achieve superior performance among various downstream tasks (6.2\% gains on classification and 2.1\% gains on detection).
%
We believe our active learning framework and Bamboo is essential for future work.
%
Code and dataset are available at \url{https://github.com/ZhangYuanhan-AI/Bamboo}.
% and continually on a comprehensive label system.
% Specifically, we contribute \textbf{\Datasetname~Dataset}, a mega-scale and information-dense dataset for both classification and detection. 
% It is built upon this human-machine synergy with two appealing properties:
% \textbf{1) Label System:} we integrate categories from 24 public datasets and collect \WikiLabelNum~new categories from knowledge bases, forming a hierarchical label system with \AllLabelNum~categories. 
% The label system is easily extendable under our designed hierarchy, and its concepts are further distinguished as ``visual'' or ``non-visual''.
% \textbf{2) Active Annotation:} based on a real-world data pool of 370M raw images crawled by the label system, only informative samples are selected for manual labeling through our human-machine active annotation framework.
% We find that rectifying out-of-distribution samples is crucial for active learning to function in realistic scenarios.
% %
% \Datasetname~aims to populate these comprehensive categories with \ClsTotalNum~image classification annotations and \DetTotalNum~object bounding box annotations. 
% %
% Compared to ImageNet22K and Objects365, models pre-trained on \Datasetname~achieve superior performance among various downstream tasks (6.2\% gains on classification and 2.1\% gains on detection).
% In addition, we provide valuable observations regarding large-scale pre-training from over 1,000 experiments.
% Due to its scalable nature on both label system and annotation pipeline, Bamboo will continue to grow and benefit from the collective efforts of the community, which we hope would pave the way for more general vision models. Bamboo are available at \hyperlink{https://opengvlab.shlab.org.cn/home}{https://opengvlab.shlab.org.cn/home}.
% \vspace{-10pt}
\keywords{Vision Dataset, Human-Machine Synergy}


\end{abstract}


==> sections/9.Rebuttal.tex <==
\begin{document}

\noindent \large{\textbf{[Response to Reviewer \#1]}} \\
\normalsize
\noindent \textbf{Q1:``The visual datasets should not be hierarchical."} \\
\noindent \noindent \textbf{A1:} 
% 1. 层次结构给超大量级的标签提供了一种合理的组成形式，虽然这样的组成形式的确存在一些如你所述的不完美的现象，但是这样的组成形式对后续研究者的使用会带来很大的便利以及新的insights。 1)很大的便利: 有层级结构, ImageNet1k作为一个benchmark可以快速的挑选出一些Mutually-exclusive的语义标签, 比如决定是保留狗还是狗的子节点作为benchmark的class,没有层级结构，我们很难快速在21K个标签中找到哪些标签的语义可能与''dog''Mutually-exclusive；拥有层级结构，用户也可以根据使用的场景挑选需要的图片用于下一步的使用，比如收集 植物 动物 地点的图片。没有层级结构，想快速收集特定语义场景的图片也比较困难。 2）新的insights：利用层级结构，许多researchers也可以开展一些研究，比如shiXXX et.al利用层级结构探索了assessing the robustness of models to subpopulation shift。
% The hierarchical structure is important for the construction of Bamboo and further research. \textbf{(1)} \textit{Dataset Construction:} As mentioned in Sec.2.2, both solution 2 and 3 require the hierarchical structure to integrate numerous concepts from the web.  \textbf{(2)} \textit{Further Research:} 
% % Without collecting labels/concepts systematically at first, it is tough to conduct further steps to improve the visual datasets. 
% Firstly, building a valid benchmark from dataset, \eg, building ImageNet1K from ImageNet, requires a hierarchical structure. Finding a group of mutually-exclusive semantic concepts to form a reasonable benchmark isn't easy. With a hierarchical structure, we can either retain an inner node and discard its whole hypernyms and hyponyms or directly pick a leaf node to achieve this goal. 
% %
% Beyond that, ~\cite{santurkar2020breeds} leverages hierarchical structure to assess the robustness of models to sub-population shift. 
% % and \cite{wen2022can} proposes that leveraging super-classes improve the accuracy of fine-grain classification.
%
Admittedly, the usage of hierarchy as semantic supervisions is debatable. \textbf{1)} Here, we mainly employ hierarchy as a tool to integrate multiple data sources. As indicated in Sec.2.2, both solutions 2 and 3 require the hierarchical structure to integrate numerous concepts from the web. \textbf{2)} We agree with R1 that ImageNet1K is built from the original ImageNet by finding a group of mutually-exclusive semantic concepts facilitated by a hierarchical structure. Similarly, we can also use hierarchy to either retain an inner node and discard its whole hypernyms and hyponyms or directly pick a leaf node to build a concise version of Bamboo. We will discuss more on hierarchy in our final version.

\noindent \textbf{Q2:``actively and continually is not a good idea..."} \\
\noindent \textbf{A2:} 
% Many popular datasets, \eg, ImageNet, are continually growing.~\cite{dehghani2021benchmark} calls for the living benchmark since the research landscape evolves. 
%
Thanks for the suggestion! We plan to release a fixed version of Bamboo to academia. Bamboo's continual nature (with infrequent version updates) aims to support new vision explorations like the enrichment of massive tail categories or the evolution of visual concepts. 

\noindent \textbf{Q3:``concern for copyright..."} \\
\noindent\textbf{A3:} Copyright and privacy are our top priority when building the dataset. \textbf{1)} 100\% images in Bamboo-DET and 40\% images in Bamboo-CLS are collected under the CC-BY license. \textbf{2)} For images not under the CC-BY license or with explicit faces, we obtain the distribution consent through official email to their creators.

\noindent \textbf{Q4:``puts the related work in the supplemental.."} \\
\noindent\textbf{A4:} Sorry for the confusion due to the space limit. We will include the related work section and the copyright/ethical discussions in the main paper.

\noindent \textbf{Q5:``this dataset is so large..."} \\
\noindent\textbf{A5:} 
% A large and public dataset is crucial for pushing academic research because similar magnitude datasets are not open source. Meanwhile, we plan to build a core set of Bamboo to help most academic research groups.
We believe a large-scale dataset could help push the boundary of computer vision research. \textbf{1)} Since existing datasets with mega-scale are private, the release of Bamboo will be a good addition for the community to discover new research questions and ideas. \textbf{2)} To democratize the usage of Bamboo, we also plan to build a concise version so that it is accessible to most academic labs.

\noindent \textbf{Q6:``other concerns..."} \\
\noindent\textbf{A6:} \textbf{1)} We plan to add mask annotations in the future version of Bamboo. \textbf{2)} "...3 out of 5 annotators" is a criterion that aims to balance the budget and quality of the annotation. \textbf{3)} As reported in ~\cite{abnar2021exploring}, by scaling up the upstream dataset, the downstream performance on several existing datasets starts to saturate. We expect the effectiveness of Bamboo could be more announced on a more comprehensive suite of downstream benchmarks.
% may be a more comprehensive set of downstream tasks that can prove the superior of Bamboo.



\noindent\large{\textbf{[Response to Reviewer \#2]}} \\
\normalsize
% We sincerely thank the appreciation of our work! \\
\noindent \textbf{Q1:``concern about collection of raw data..."} \\
\noindent\textbf{A1:} Please refer to A3 to R1 for the detailed explanation.

\noindent \textbf{Q2:``Additional comments "} \\
\noindent\textbf{A2:} \textbf{1)} Thank you for the advice! We will credit these datasets in Sec.2.1 in our final version.. \textbf{2)} We have 700 annotators each for Bamboo-CLS and Bamboo-DET. The total annotation hours are 167,000 and 23,000, respectively. \textbf{3)} Yes, we plan to include more unsupervised methods on Bamboo to form a comprehensive comparison.



\noindent\large{\textbf{[Response to Reviewer \#3]}} \\
\normalsize
\noindent\textbf{Q1:``give the annotation accuracy"} \\
\noindent\textbf{A1:} \textbf{1)} We check the annotation accuracy by employing another quality control team. Specifically, they randomly select 10\% annotations to inspect the annotation quality. The average annotation accuracy is 91.21\% for Bamboo-CLS and 88.67\% for Bamboo-DET.


\noindent\textbf{Q2:``List of the 24 datasets...datasets for downstream..."} \\
\noindent\textbf{A2:} Sorry for the confusion. Specifically, the 12 datasets used for downstream evaluation are shown in Table 2, 3 in the main paper, while the 12 datasets used for upstream pre-training are described in lines 452-455 and 466 of the supplementary material. 
% These 24 datasets are the components of our label system.



\noindent\large{\textbf{[Response to Reviewer \#4]}} \\
\normalsize
\noindent\textbf{Q1:``...to write this paper would be to focus on..."} \\
\noindent\textbf{A1:} Thank you for the advice!  \textbf{1)} We introduce the detailed statistics of Bamboo in Fig.3 of supplementary material. \textbf{2)} We construct the current ontology based on mainly two considerations: (a) integrating the current dataset concepts into WordNet using solution 1,3,4, (b) finding more concepts to enrich our ontology by our proposed solution 2. 
% We are looking forward to other good solutions. Welcome to share new suggestions!  
\textbf{3)} 
% The practical solutions to building an extensive labeling system and conducting an effective active learning annotation make Bamboo different from prior works. Therefore, we think they may deserve a detailed description. 
Different from prior works, Bamboo is built upon a semantically-informed label system and an active annotation process. These designs aim to provide a complete coverage of visual categories while balancing between annotation accuracy and efficiency.

% \noindent\textbf{Q2:``"} \\
% \noindent\textbf{A2:} Even though Bamboo is the most significant contribution of this paper, the process of constructing Bamboo, including the labeling system and the active learning, makes Bamboo different from the prior works and are valuable for researchers to develop datasets in another domain. We believe this process deserves to be detailed in the main paper.  


% \noindent\textbf{Q3:``why the ontology is merged in a current way"} \\
% \noindent\textbf{A3:} 

\noindent\textbf{Q2:``...typos and writing''.} \\
\noindent\textbf{A2:} We apologize for the typos. We will carefully revise them and polish the paper in our final version. 

\noindent\textbf{Q3:``Some clarification...higher-level questions''} \\
\noindent\textbf{A3:} \textbf{1)} Yes, the knowledge base is Wikipedia. \textbf{2)} As indicated in lines 797-809, the experimental results validate the effectiveness of our label system in Bamboo compared to ImageNet. \textbf{3)} Each image only has a single label. \textbf{4)} By leveraging WordNet, most overlapping categories can be classified into a single synset. Line 233-238 in the main paper also describes a solution to address the overlapping categories. \textbf{5)} We ask the annotators to only select images with a dominant category. \textbf{6)} The duplicated images are removed in the post-processing.

\noindent\textbf{Q4:``Why does not release the dataset...''} \\
\noindent\textbf{A4:} 
% Releasing a dataset requires numerous preparing works, 
% including building a website, finding a space to store the dataset, etc., 
% and all of these works need time to conduct. We will release our dataset as soon as possible. 
Yes, we do plan to release the dataset soon. We will set up a website to host and showcase the ontology as well as images under each category. The CVPR committee also has a rigorous process to check the dataset release status.

\vspace{-10pt}
\end{document}
